Characterizing multiple instance datasets

In many pattern recognition problems, a single feature vector is not sufficient to describe an object. In multiple instance learning (MIL), objects are represented by sets (\emph{bags}) of feature vectors (\emph{instances}). This requires an adaptation of standard supervised classifiers in order to train and evaluate on these bags of instances. Like for supervised classification, several benchmark datasets and numerous classifiers are available for MIL. When performing a comparison of different MIL classifiers, it is important to understand the differences of the datasets, used in the comparison. Seemingly different (based on factors such as dimensionality) datasets may elicit very similar behaviour in classifiers, and vice versa. This has implications for what kind of conclusions may be drawn from the comparison results. We aim to give an overview of the variability of available benchmark datasets and some popular MIL classifiers. We use a dataset dissimilarity measure, based on the differences between the ROC-curves obtained by different classifiers, and embed this dataset dissimilarity matrix into a low-dimensional space. Our results show that conceptually similar datasets can behave very differently. We therefore recommend examining such dataset characteristics when making comparisons between existing and new MIL classifiers. The datasets are available via Figshare at \url{https://bit.ly/2K9iTja}.

==> miltable.tex <==
\begin{tabular}{c l c r r}
  nr&  name                     &+/- bags  & inst  & dim \\
\hline
 101& Musk 1                    &47/45    &     476 &  166 \\
 102& Musk 2                    &39/63    &    6598 &  166 \\
 103& Artificial Gaussian       &10/10    &   +-150 &    2 \\
 104& Artificial Maron          &10/10    &   -1000 &    2 \\
 105& Surrey Cathedral          & 5/3476  &   96869 &   33 \\
 106& Artificial Concept        &10/10    &   +-150 &    2 \\
 107& Artificial Difficult      &10/40    &     350 &    2 \\
 108& Artificial Rotated        &30/30    &    1355 &    2 \\
 109& Artificial Widened        &30/30    &    1320 &    2 \\
 110& Corel African             &00/1900  &    7947 &    9 \\
 111& Corel Beach               &00/1900  &    7947 &    9 \\
 112& Corel Historical          &00/1900  &    7947 &    9 \\
 113& Corel Buses               &00/1900  &    7947 &    9 \\
 114& Corel Dinosaurs           &00/1900  &    7947 &    9 \\
 115& Corel Elephants           &00/1900  &    7947 &    9 \\
 116& Corel Flowers             &00/1900  &    7947 &    9 \\
 117& Corel Horses              &00/1900  &    7947 &    9 \\
 118& Corel Mountains           &00/1900  &    7947 &    9 \\
 119& Corel Food                &00/1900  &    7947 &    9 \\
 120& Corel Dogs                &00/1900  &    7947 &    9 \\
 121& Corel Lizards             &00/1900  &    7947 &    9 \\
 122& Corel Fashion             &00/1900  &    7947 &    9 \\
 123& Corel Sunset              &00/1900  &    7947 &    9 \\
 124& Corel Cars                &00/1900  &    7947 &    9 \\
 125& Corel Waterfalls          &00/1900  &    7947 &    9 \\
 126& Corel Antique             &00/1900  &    7947 &    9 \\
 127& Corel Battleships         &00/1900  &    7947 &    9 \\
 128& Corel Skiing              &00/1900  &    7947 &    9 \\
 129& Corel Desserts            &00/1900  &    7947 &    9 \\
 130& SIVAL AjaxOrange          &60/1440  &   47414 &   30 \\
 131& SIVAL Apple               &60/1440  &   47414 &   30 \\
 132& SIVAL Banana              &60/1440  &   47414 &   30 \\
 133& SIVAL BlueScrunge         &60/1440  &   47414 &   30 \\
 134& SIVAL CandleWithHolder    &60/1440  &   47414 &   30 \\
 135& SIVAL CardboardBox        &60/1440  &   47414 &   30 \\
 136& SIVAL CheckeredScarf      &60/1440  &   47414 &   30 \\
 137& SIVAL CokeCan             &60/1440  &   47414 &   30 \\
 138& SIVAL DataMiningBook      &60/1440  &   47414 &   30 \\
 139& SIVAL DirtyRunningShoe    &60/1440  &   47414 &   30 \\
 140& SIVAL DirtyWorkGloves     &60/1440  &   47414 &   30 \\
 141& SIVAL FabricSoftenerBox   &60/1440  &   47414 &   30 \\
 142& SIVAL FeltFlowerRug       &60/1440  &   47414 &   30 \\
 143& SIVAL GlazedWoodPot       &60/1440  &   47414 &   30 \\
 144& SIVAL GoldMedal           &60/1440  &   47414 &   30 \\
 145& SIVAL GreenTeaBox         &60/1440  &   47414 &   30 \\
 146& SIVAL JuliesPot           &60/1440  &   47414 &   30 \\
 147& SIVAL LargeSpoon          &60/1440  &   47414 &   30 \\
 148& SIVAL RapBook             &60/1440  &   47414 &   30 \\
 149& SIVAL SmileyFaceDoll      &60/1440  &   47414 &   30 \\
 150& SIVAL SpriteCan           &60/1440  &   47414 &   30 \\
 151& SIVAL StripedNotebook     &60/1440  &   47414 &   30 \\
 152& SIVAL TranslucentBowl     &60/1440  &   47414 &   30 \\
 153& SIVAL WD40Can             &60/1440  &   47414 &   30 \\
 154& SIVAL WoodRollingPin      &60/1440  &   47414 &   30 \\
 155& Web recommendation user 1 &17/58    &   2212  & 5863 \\
 156& Web recommendation user 2 &18/57    &   2212  & 6519 \\
 157& Web recommendation user 3 &14/61    &   2212  & 6306 \\
 158& Web recommendation user 4 &55/20    &   2291  & 6059 \\
 159& Web recommendation user 5 &61/14    &   2546  & 6407 \\
 160& Web recommendation user 6 &59/16    &   2462  & 6417 \\
 161& Web recommendation user 7 &39/36    &   2400  & 6450 \\
 162& Web recommendation user 8 &35/40    &   2183  & 5999 \\
 164& Newsgroup alt.atheism     &50/50    &   5443  &  200 \\
 165& Newsgroup comp.graphics   &49/51    &   3094  &  200 \\
 166& comp.os.ms-windows.misc   &50/50    &   5175  &  200 \\
 167& comp.sys.ibm.pc.hardware  &49/51    &   4827  &  200 \\
 168& comp.sys.mac.hardware     &50/50    &   4473  &  200 \\
 169& comp.windows.x            &49/51    &   3110  &  200 \\
 170& misc.forsale              &50/50    &   5306  &  200 \\
 171& rec.autos                 &50/50    &   3458  &  200 \\
 172& rec.motorcycles           &50/50    &   4730  &  200 \\
 173& rec.sport.baseball        &50/50    &   3358  &  200 \\
 174& rec.sport.hockey          &50/50    &   1982  &  200 \\
 175& sci.crypt                 &50/50    &   4284  &  200 \\
 176& sci.electronics           &47/53    &   3192  &  200 \\
 177& sci.med                   &50/50    &   3045  &  200 \\
 178& sci.space                 &50/50    &   3655  &  200 \\
 179& soc.religion.christian    &50/50    &   4677  &  200 \\
 180& talk.politics.guns        &50/50    &   3558  &  200 \\
 181& talk.politics.mideast     &50/50    &   3376  &  200 \\
 182& talk.politics.misc        &50/50    &   4788  &  200 \\
 183& talk.religion.misc        &49/51    &   4606  &  200 \\
 201&300. COIL100       between &08-1301  &  48004  &   32 \\
 301& Fox                       &100/100  &   1302  &  230  \\
 302& Tiger                     &100/100  &   1220  &  230  \\
 303& Elephant                  &100/100  &   1391  &  230  \\
 304& TREC9 (pretest) 1         &200/200  &   3224  &66552 (31 non-zero)
 \\
 305& TREC9 (pretest) 2         &200/200  &   3344  &66153 (31) \\
 306& TREC9 (pretest) 3         &200/200  &   3246  &66144 (31) \\
 307& TREC9 (pretest) 4         &200/200  &   3391  &67085 (32) \\
 308& TREC9 (pretest) 7         &200/200  &   3365  &66823 (31) \\
 309& TREC9 (pretest) 9         &200/200  &   3300  &66627 (33) \\
 310& TREC9 (pretest) 10        &200/200  &   3453  &66082 (32) \\
 311& Harddrive, pos = normal   &178/191  &   68411 &   61 (or 59, 2
 features might be meta-data) \\
 312& Harddrive, pos = failure  &191/178  &   68411 &   61 (or 59, 2
 features might be meta-data) \\
 313& Trx protein family        &25/168   &   26611 &    8   \\
 314& Mutagenesis easy          &125/63   &   10486 &    7  \\
 315& Mutagenesis hard          &13/29    &    2132 &    7 \\
 316& Brown Creeper             &197/351  &   10232 &   38  \\
 317& Winter Wren               &109/439  &   10232 &   38  \\
 318& Pacific slope Flycatcher  &165/383  &   10232 &   38  \\
 319& Red-breasted Nuthatch     &82/466   &   10232 &   38  \\
 320& Dark-eyed Junco           &20/528   &   10232 &   38  \\
 321& Olive-sided Flycatcher    &90/458   &   10232 &   38  \\
 322& Hermit Thrush             &15/533   &   10232 &   38  \\
 323& Chestnut-backed Chickadee &117/431  &   10232 &   38  \\
 324& Varied Thrush             &89/459   &   10232 &   38  \\
 325& Hermit Warbler            &63/485   &   10232 &   38  \\
 326& Swainsons Thrush          &79/469   &   10232 &   38  \\
 327& Hammonds Flycatcher       &103/445  &   10232 &   38  \\
 328& Western Tanager           &46/502   &   10232 &   38  \\
 329& Biocreative Component     &359/359  &13129/23765 & 200 \\
 330& Biocreative Function      &385/385  &13498/42038 & 200 \\
 331& Biocreative Process       & 620/620 &21306/97111 & 200 \\
 332& UCSB breast cancer        & 26/32   &    2002 &   708  \\
 333& Messidor retinopathy      &654/546  &    12352&   687 \\
\end{tabular} 

